A Practitioner's Guide to Continual Multimodal Pretraining

Multimodal foundation models serve numerous applications at the intersection of vision and language. Still, despite being pretrained on extensive data, they become outdated over time. To keep models updated, research into continual pretraining mainly explores scenarios with either (1) infrequent, indiscriminate updates on large-scale new data, or (2) frequent, sample-level updates. However, practical model deployment often operates in the gap between these two limit cases, as real-world applications often demand adaptation to specific subdomains, tasks or concepts -- spread over the entire, varying life cycle of a model. In this work, we complement current perspectives on continual pretraining through a research test bed as well as provide comprehensive guidance for effective continual model updates in such scenarios. We first introduce FoMo-in-Flux, a continual multimodal pretraining benchmark with realistic compute constraints and practical deployment requirements, constructed over 63 datasets with diverse visual and semantic coverage. Using FoMo-in-Flux, we explore the complex landscape of practical continual pretraining through multiple perspectives: (1) A data-centric investigation of data mixtures and stream orderings that emulate real-world deployment situations, (2) a method-centric investigation ranging from simple fine-tuning and traditional continual learning strategies to parameter-efficient updates and model merging, (3) meta learning rate schedules and mechanistic design choices, and (4) the influence of model and compute scaling. Together, our insights provide a practitioner's guide to continual multimodal pretraining for real-world deployment. Our benchmark and code is here: https://github.com/ExplainableML/fomo_in_flux.

==> benchmark.tex <==
\section{The FoMo-in-Flux Benchmark}

% Adapt Table
\begin{table}[ht]
\centering
\caption{Adapt datasets and their properties. Eval datasets and their properties.}

\begin{minipage}[t]{0.495\textwidth}
\resizebox{\linewidth}{!}{
 \begin{tabular}{lcccc}
\toprule
Dataset & \#Train & \#Test & \#Classes \\
\midrule
\multicolumn{4}{l}{\textbf{classification-based}} \\
ai2diagrams & 2720 & 681 & 15 \\
artbench10 & 47531 & 11883 & 1870 \\
birdsnap & 31905 & 7977 & 500 \\
cifar100 & 50000 & 10000 & 100 \\
clevr & 55931 & 13983 & 217 \\
clrs & 13525 & 1475 & 25 \\
country211 & 31650 & 21100 & 211 \\
cub200 & 5994 & 5794 & 200 \\
df20mini & 32724 & 3637 & 179 \\
dollarstreet & 13555 & 4103 & 1701 \\
domainnet\_clipart & 33525 & 14604 & 345 \\
domainnet\_infograph & 36023 & 15582 & 345 \\
domainnet\_painting & 50416 & 21850 & 344 \\
domainnet\_sketch & 48212 & 20916 & 345 \\
dsprites & 75000 & 25000 & 27 \\
dtd & 1880 & 1880 & 47 \\
fgvcaircraft & 3334 & 3333 & 100 \\
flowers102 & 6149 & 1020 & 102 \\
fru92 & 55814 & 9200 & 92 \\
inaturalist2021 & 125000 & 25000 & 2500 \\
isicmelanoma & 2245 & 562 & 7 \\
mitstates & 43002 & 10751 & 1959 \\
mtsd & 59978 & 8737 & 227 \\
mvtecad\_adapt & 2903 & 726 & 15 \\
mvtecad\_eval & 1380 & 345 & 88 \\
objectnet & 40134 & 10000 & 313 \\
obsc\_animals & 17000 & 4238 & 74 \\
obsc\_things & 19128 & 4758 & 84 \\
openimages & 115333 & 8593 & 589 \\
patternnet & 26600 & 3800 & 38 \\
places365 & 120231 & 36499 & 365 \\
plantvillage & 43444 & 10681 & 38 \\
quilt & 95862 & 23966 & 157 \\
resisc45 & 18900 & 6300 & 45 \\
shapes3d & 75000 & 25000 & 864 \\
snake\_clef & 151031 & 14117 & 1599 \\
sun397 & 15880 & 19850 & 397 \\
synthclip106 & 84800 & 13886 & 106 \\
veg200 & 61117 & 20000 & 200 \\
zappos50k & 37829 & 9458 & 1847 \\
\midrule
\multicolumn{4}{l}{\textbf{retrieval-based}} \\
fscoco (avg T2I/I2T R@5) & 7105 & 1777 & 115 \\
\bottomrule
\end{tabular}}
\label{tab:adapt-datasets}
\end{minipage}
\begin{minipage}[t]{0.495\textwidth}
\resizebox{\linewidth}{!}{
   \begin{tabular}{lcccc}
\toprule
Dataset & \# Train & \# Test & \# Classes \\
\midrule
\multicolumn{4}{l}{\textbf{classification-based}} \\
caltech101 & 6026 & 2651 & 101 \\
caltech256 & 21307 & 9300 & 257 \\
cars196 & 8144 & 8041 & 196 \\
cifar10 & 50000 & 10000 & 10 \\
country211 & 31650 & 21100 & 211 \\
cub200 & 5994 & 5794 & 200 \\
domainnet\_quickdraw & 60375 & 25875 & 345 \\
eurosat & 18900 & 8100 & 10 \\
fashionmnist & 60000 & 10000 & 10 \\
food101 & 75750 & 25250 & 101 \\
gtsrb & 18635 & 8005 & 43 \\
imagenet & 0 & 50000 & 1000 \\
imagenet\_a & 0 & 7500 & 200 \\
imagenet\_d & 0 & 4835 & 103 \\
imagenet\_r & 0 & 30000 & 200 \\
imagenet\_s & 0 & 50889 & 1000 \\
imagenet\_v2 & 0 & 10000 & 1000 \\
mnist & 60000 & 10000 & 10 \\
monkeys10 & 1097 & 272 & 10 \\
oxford\_pets & 3680 & 3669 & 37 \\
stl10 & 5000 & 8000 & 10 \\
svhn & 73257 & 26032 & 10 \\
\midrule
\multicolumn{4}{l}{\textbf{retrieval-based}} \\
mscoco (avg T2I/I2T R@5) & 0 & 5000 & 0 \\
flickr30k (avg T2I/I2T R@5) & 0 & 1000 & 0 \\
\bottomrule
\end{tabular}}
\label{tab:eval-datasets} 
\end{minipage}
\end{table}


\textbf{Creation.}

\textbf{Experimental Details.}
\begin{itemize}
    \item \textbf{CLIP models used. } On huggingface, the CLIP models that were downloaded the most were CLIP ViT-B-32-laion2b (6.11M times), CLIP-ViT-H-14-laion2b (4M times), and CLIP-ViT-B-16 (2M times). Hence, we investigate these three models. But ofcourse, not all general practitioners use ViT-H-14 since it needs way more compute resources. Hence, we focus on ViT-B-32 and ViT-B-16 in our study. On top of that ViT-B/16 has been used in other studies such as TiC-CLIP.
    \item \textbf{Datasets used.}
    \item \textbf{Optimisation algorithms.}
    \item \textbf{Continual Pretraining Task itself is practicall relevant.}
\end{itemize}

\textbf{Approaches for Continually Updating Models.}

\textbf{Evaluation of Adaptation and Downstream Generalization.}

\textbf{Challenges.}

\clearpage

==> figures/latex_figs/capsfusion.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/capsfusion_examples.pdf}
    \caption{\textbf{PLACEHOLDER FOR CAPSFUSION PIPELINE.} Capsfusion Pipeline.}
    \label{fig:capsfusion-caps}
\end{figure}

==> figures/latex_figs/dataorderings.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/data_streams_full_finetune_vit_b16_numtasks20.pdf}
    \caption{\textbf{Effect of the data-stream ordering $\pi$}}
    \label{fig:data-centric-stream-orderings-pareto-frontier}
\end{wrapfigure}

==> figures/latex_figs/merge_data.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.47\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/data_mixing_ratios_random_data_stream_vit_b16_numtasks20.pdf}
    \vspace{-14pt}
    \caption{\textbf{Different Data Mixture Ratios} $\lambda_{\mathcal{D}/\mathcal{P}/\mathcal{B}}$ between pretraining $\mathcal{P}$, update $\mathcal{D}$ and buffer pool $\mathcal{B}$ yield significantly different adaptation-retention behaviour.}
    \label{fig:data-mixing-ratios-ablation}
    \end{subfigure}
    \begin{subfigure}[b]{0.47\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/pretraining_data_pool_random_data_stream_vit_b16_numtasks20.pdf}
    \vspace{-18pt}
    \caption{\textbf{Quality and Diversity of the Pretraining Pool} $\mathcal{P}$ can matter significantly for retention of initial zero-shot performance.}
    \label{fig:pretraining-data-pool-ablation}
    \end{subfigure}
\caption{\textbf{Study on Mixture Ratios and Pretraining Pools.}}
\end{figure}

